CRAG-MM-Diagnostics: Enabling Stage-Wise Analysis of Knowledge-Intensive VQA

Knowledge-Intensive Visual Question Answering (KI-VQA) benchmarks evaluate Vision-Language Models (VLMs) as multimodal knowledge assistants by requiring external information beyond a provided image to answer questions. KI-VQA involves multiple sub-problems -referring expression understanding, visual grounding, object recognition, knowledge retrieval, and reasoning-yet existing benchmarks typically report only end-task accuracy, obscuring where failures arise. To analyze the full KI-VQA pipeline, we introduce CRAG-MM-Diagnostics, a diagnostic benchmark with stage-wise data annotations that isolate 1) language-based visual grounding, 2) object identification, and 3) knowledge retrieval and reasoning. We evaluate fully parametric and retrieval-augmented VLMs, providing fine-grained analyses using newly collected metadata, such as target ROIs, entity names, and visual complexity scores. Our results point to knowledge retrieval and reasoning as the primary bottleneck, but also highlight issues in the other parts of the KI-VQA pipeline, such as the fact that VLMs struggle with target object identification or that image retrievers struggle to integrate textual cues. These findings expose fundamental limitations in current KI-VQA systems and motivate stage-aware evaluation. We, lastly, leverage these findings to propose a grounded bimodal RAG pipeline that integrates a visual grounding module to crop targets before image retrieval, boosting GPT-5 and Qwen's respective accuracies by 13.3 and 8.5 percentage points.

==> Tables/KnowledgeExtraction_decoupled_analysis.tex <==
\begin{table}[h!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccc}
\toprule
Image & Query & Llama 11b & Qwen 3b & Qwen 7b \\
\midrule
Original & Original & 12 & 8 & 10 \\
Easy Image & Original (minor edited referring) & 16 & 10 & 12 \\
X & Original (textual only) & 34 & 16 & 24 \\
Original & Easy Recognition query & 38 & 24 & 38 \\
Easy Image & Easy Recognition query & 64 & 50 & 58 \\
\bottomrule
\end{tabular}
}
\caption{Decoupled analysis of diagnosing bottleneck of VLMs.}
\label{tab:knowledgeExtraction_decoupled_analysis}
\end{table}



==> Tables/imageRetriever_performance.tex <==
\begin{table}[h!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lllll}
\toprule
Retriever Type & \multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Recall@1}} & \multicolumn{1}{c}{\textbf{Recall@5}} & \multicolumn{1}{c}{\textbf{Recall@10}} \\
\toprule
proprietary & GoogleLens & 46.0 & 50.0 & 54.0 \\
Unimodal & CLIP-ViT & 14.0 & 22.0 & 30.0 \\
Advanced & CLIP-ViT + Cropping (Qwen7B) & 24.0 & 38.0 & 40.0 \\
Advanced & CLIP-ViT + Cropping (GPT-4.1) & 28.0 & 40.0 & 44.0 \\
Advanced & CLIP-ViT + Cropping (GT) & 20.0 & 36.0 & 46.0 \\
Multimodal & VLM2VEC-v2.0 & 2.0 & 10.0 & 10.0 \\
\bottomrule
\end{tabular}
}
\caption{Image retriever performance per diverse retrievers. \hs{will be updated with new datasets}}
\label{tab:imageRetriever_performance}
\end{table}


==> Tables/knoweldge_intensive_questionAnswering_performance.tex <==
\begin{table*}[t!]
\small
\caption{
Comparison of (a) generalized and (b) RAG models, evaluated using KI-VQA end-task accuracy.
\textit{All} reports performance over all test instances, while \textit{Subset} evaluates examples with ambiguous referring expressions.
\textit{txt-only} is an ablation during which we evaluate using questions with the gold entity name inserted, whereas \textit{txt+img} is the conventional KI-VQA setup.
The shaded row uses groundtruth target regions for visual grounding.
}
\vspace{-0.35cm}
\label{table:knowledge_intensive_qa}

\renewcommand{\arraystretch}{1.2}
\begin{subtable}[t]{0.47\textwidth}
\caption{Generalized models \parishad{Figure wip}}

\begin{adjustbox}{width=\linewidth}
\begin{tabular}{@{} l c *{4}{S} @{}}
\toprule
\multicolumn{2}{c}{\textit{Model}} & \multicolumn{2}{c}{\textit{All}} & \multicolumn{2}{c}{\textit{Subset}} \\
\cmidrule(lr){1-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}
& & {\rotatebox[origin=c]{90}{\scriptsize txt+img}}
  & {\rotatebox[origin=c]{90}{\scriptsize txt-only}}
  & {\rotatebox[origin=c]{90}{\scriptsize ambig.}}
  & {\rotatebox[origin=c]{90}{\scriptsize dis.}} \\
\midrule
\texttt{Llama} & 11B & 25.3 & 29.2 & 22.4 & 21.0 \\
\addlinespace[1pt]
\multirow{4}{*}{\texttt{Qwen}}
  & 3B  & 18.7 & 25.0 & 18.4 & 17.7 \\
  & 7B  & 20.4 & 30.1 & 16.8 & 16.9 \\
  & 32B & 26.2 & 34.9 & 22.4 & 28.2 \\
  & 72B & \bfseries 31.4 & \bfseries 42.6 & \bfseries 24.8 & \bfseries 30.7 \\
\addlinespace[1pt]
\texttt{GPT-5-mini} & {-} & 40.2 & 50.5 & 34.4 & 36.0 \\
\texttt{GPT-5}      & {-} & \bfseries 48.3 & \bfseries 58.8 & \bfseries 44.0 & \bfseries 45.6 \\
\bottomrule
\end{tabular}
\label{tab:performance_baseline}
\end{adjustbox}
\end{subtable}
\hfill
\begin{subtable}[t]{0.47\textwidth}
\caption{RAG models}

  \renewcommand{\arraystretch}{0.9}
\begin{adjustbox}{width=\linewidth}
\input{ECCV/Tables/stage3_ablations}
\label{tab:performance_rag}
\end{adjustbox}
\end{subtable}

\vspace{-0.15cm}
\label{tab:end-task-accuracy}
\end{table*}

==> Tables/objectIdentification_complexity_analysis.tex <==
\begin{table}[h!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l l l c c}
\toprule
\textbf{Setting} & \textbf{Image} & \textbf{Query} & \textbf{Qwen-7B} & \textbf{GPT-4.1} \\
\midrule
Type1 & Original & Original & 44.0 & 52.0 \\
Type2 & Cropped & Recognition & 32.0 & 60.0 \\
Type3 & BBox & Original & 42.0 & 52.0 \\
Type4 & BBox & Recognition & 26.0 & 38.0 \\
\bottomrule
\end{tabular}
}
\caption{Effect of query and image simplification on object identification accuracy in CRAG-MM (50 examples).
Type1: original image + original query.
Type2: cropped image + recognition query.
Type3: image with bounding box + original query.
Type4: image with bounding box + recognition query.}
\label{tab:objectIdentification_complexityOfQuery}
\end{table}


==> Tables/objectIdentification_overall_performance.tex <==
\begin{table*}[t]
  \caption{
  Target Object Identification. Comparison of \textbf{Gen}eralized and \textbf{Spec}ialized models on the target object identification task: given an image, the model must retrieve the correct entity name of the target object.
  \textbf{All} reports performance over all test instances, while \textbf{Subset} evaluates over a subset from \textsc{ORI./Q-Y} setup, where the queries are \textbf{Ambig}uous and when we \textbf{Dis}ambiguate the question.
  Under \textbf{All}, \textbf{Crop}/\textbf{Ori.} indicates whether the input image is cropped to the grounded target object (after ground truth target object grounding) or the original full image is used. 
  \textbf{Q-Y} and \textbf{Q-N} denote whether the text query is provided or not to the model, respectively. 
  For the retrieval models, results are reported as top-1 (left) and top-10 (right). \hs{for gen. models image is not highlighted not cropped, for sepc. models image is cropped. need to elaborate}
  }
  \label{table:object_identification}
  \begin{center}
    \begin{small}
      \begin{sc}
        \begin{tabular}{lcc|cccc|cc}
          \toprule
          & & & \multicolumn{4}{c}{All} & \multicolumn{2}{c}{Subset} \\
          \midrule
          & Model  & Size  & Ori./Q-Y & Crop/Q-Y & Ori./Q-N & Crop/Q-N& Ambig. & Dis. \\
          \midrule
          \multirow{7}{*}{Gen} 
          & Llama & 11B & 38.7 & 39.5  & 28.8 & 33.2 & 29.6 & 40.0\\
          \cmidrule{2-9}
          & \multirow{4}{*}{Qwen} 
                & 3B & 35.3  & 38.1 & 27.6 & 31.6 & 28.8 & 36.8\\
                && 7B & 40.6 & 42.9 & 32.5  & 35.0&  32.8 & 39.2  \\
                && 32B & 44.0 & 42.0 & 35.7 & 36.7&  38.4 & 37.6 \\
                && 72B & 52.1  & 52.0 & 40.1 & 45.2& 44.0 & 48.0\\
          \cmidrule{2-9}
          & GPT-5-mini &  & 54.4 & 52.48  & 35.7 & 37.86 & 47.2 & 59.2\\
          & GPT-5 &  & 60.31 & 46.39  & 39.0 & 31.07 & 58.4 & 63.2\\
          \midrule
          \multirow{3}{*}{Spec} 
          & CLIP-VIT & 0.4B & - & - & 15.0/31.9 & 20.2/41.8 & - & - \\
          & VLM2VECv2-Qwen2VL & 7B & 8.9/20.5 & 9.4/24.1 & 12.4/26.7 & 15.8/34.4 & - & -  \\
          & Qwen-3-VL-emb & 2B & 12.6/29.8 & 18.5/36.7 & 22.1/43.0 & 31.3/51.9& - & -  \\
          
          \bottomrule
        \end{tabular}
      \end{sc}
    \end{small}
  \end{center}
  \vskip -0.1in
\end{table*}


==> Tables/related_works_comparison.tex <==

\begin{table*}[t]
  \small
  \centering
  \caption{TBD}
  \renewcommand{\arraystretch}{1.1}

  \begin{tabularx}{\textwidth}{
    >{\raggedright\arraybackslash}p{3.2cm}
    >{\centering\arraybackslash}p{1.6cm}
    >{\centering\arraybackslash}p{1.4cm}
    >{\centering\arraybackslash}p{1.6cm}
    >{\centering\arraybackslash}p{1.4cm}
    >{\centering\arraybackslash}p{1.6cm}
    >{\centering\arraybackslash}p{1.8cm}
  }
    \toprule
    \textbf{Dataset} &
    \textbf{\scriptsize Knowledge} &
    \textbf{\scriptsize Visual Metadata} &
    \textbf{\scriptsize Google Lens Recall@10} &
    \multicolumn{3}{c}{\textbf{Visual Difficulty}} \\
    \cmidrule(lr){5-7}
    & & & &
    {\scriptsize \textbf{Target size}} &
    {\scriptsize \textbf{Objs. per img.}} &
    {\scriptsize \textbf{Dist. from center}} \\
    \midrule
    \textbf{\scriptsize V* \citep{wu2024v}} &
    None &
    \cmarkgray &
    -- &
    Small & 9.64 & 0.48 \\
    \midrule
    \textbf{\scriptsize OK-VQA \citep{marino2019ok}} &
    {\scriptsize Commonsense} &
    \xmark &
    -- &
    Large & 7.5 & 0.19 \\
    \midrule
    \textbf{\scriptsize EncyclopedicVQA \citep{Mensink2023EncyclopedicVV}} &
    Factual &
    \xmark &
    64.00 &
    Medium & 1.2 & 0.12 \\
    \midrule
    \textbf{\scriptsize ViQuAE \citep{Lerner2022ViQuAEAD}} &
    Factual &
    \xmark &
    74.00 &
    Large & 4.9 & 0.08 \\
    \midrule
    \textbf{\scriptsize VisualSimpleQA \citep{Wang2025VisualSimpleQAAB}} &
    Factual &
    \cmark &
    56.00 &
    Medium & 5.8 & 0.28 \\
    \midrule
    \textbf{\scriptsize InfoSeek \citep{chen2023can}} &
    Factual &
    \xmark &
    63.26 &
    Large & 1.6 & 0.14 \\
    \midrule
    \textbf{\scriptsize CRAG-MM \citep{cragMM2025}} &
    Factual {\scriptsize (Partial)} &
    \cmarkgray &
    55.10 &
    Medium & 4.2 & 0.26 \\
    \midrule
    \textbf{\ours{} (Ours)} &
    Factual &
    \cmark &
    38.77 &
    Small & 8.4 & 0.30 \\
    \bottomrule
  \end{tabularx}

  \label{tab:related_works_datasets}
\end{table*}

